DriftGAN: Using historical data for Unsupervised Recurring Drift Detection

In real-world applications, input data distributions are rarely static over a period of time, a phenomenon known as concept drift. Such concept drifts degrade the model's prediction performance, and therefore we require methods to overcome these issues. The initial step is to identify concept drifts and have a training method in place to recover the model's performance. Most concept drift detection methods work on detecting concept drifts and signalling the requirement to retrain the model. However, in real-world cases, there could be concept drifts that recur over a period of time. In this paper, we present an unsupervised method based on Generative Adversarial Networks(GAN) to detect concept drifts and identify whether a specific concept drift occurred in the past. Our method reduces the time and data the model requires to get up to speed for recurring drifts. Our key results indicate that our proposed model can outperform the current state-of-the-art models in most datasets. We also test our method on a real-world use case from astrophysics, where we detect the bow shock and magnetopause crossings with better results than the existing methods in the domain.

==> content/application.tex <==
In this section, we look at an application scenario involving the magnetosphere readings of Mercury. We apply our approach to a real use case from planetary science to demonstrate the applicability as an improved sampling strategy.

\begin{figure}[ht]
    \centering
    \subfloat[\centering ]{{\includegraphics[width=5cm, height=3cm]{images/slavin_mercury.jpg} }}%
    \qquad
    \subfloat[\centering]
    {{\includegraphics[width=5cm, height = 3cm]{images/zurbuchen_messenger.jpg} }}%
     \caption[]{{(a) Schematic view of Mercury's magnetic conditions~\cite{slavin2004mercury}.The bow shock slows down the approaching solar wind to subsonic speeds. The magnetopause further acts as an obstacle.  (b) A typical MESSENGER orbit path: the spacecraft passed from
    the \emph{interplanetary magnetic field} (IMF) through bow shock, magnetosheath, magnetopause and magnetosphere regions of Mercury and then through the same sequence in reverse~\cite{zurbuchen2011messenger}. }}
    \label{fig: introduction}%
\end{figure}


The \emph{magnetosphere} of a planet is the area surrounding it where the planet's magnetic field is stronger than that of the surrounding interplanetary space. 
The \emph{magnetopause} is the outer boundary of this region, while the \emph{magnetosheath} lies above it and extends to the bow shock. 
The \emph{bow shock} is a shock wave that decelerates the solar wind and deflects it around the planet's magnetospheric cavity as shown in~\autoref{fig: introduction}.
The magnetic field of Merucury is highly variable due to its closest proximity to the sun, and a weak magnetic core. However, due to its global nature and similarity to Earth's magnetic field, it has gathered increasing attention from researchers.
To this end, NASA launched a spacecraft called MESSENGER to orbit Mercury and conduct long-term empirical studies~\cite{solomon2007messenger}. MESSENGER collected over 4000 orbits' worth of data.

We need to classify whether the spacecraft is in interplanetary space, bow shock crossing(SK), magnetosheath (MSh), magnetopause crossing(MP) or in Mercury's magnetosphere(MSp). MESSENGER spends most of its time in interplanetary space and the other events are comparatively rare as shown in \autoref{tab:labels}.
The magnetic field of Mercury is very dynamic owing to the presence of solar winds and is considerably affected by the solar activity. Therefore, identifying such events is difficult. Supervised learning typically requires a large number of samples for training but labelling all the orbits and events is extremely time-consuming and expensive as we require experts to label the data by hand. 

The dataset we use for our experiments in this work contains magnetic field measurements from the MESSENGER magnetometer instrument. The data is already preprocessed with removal of calibration signals, enrichment with Mercury position data, and split according to UTC day boundaries and Mercury apoapsis.
This cleaned and prepared dataset introduced in~\cite{julkadeep} contains 2776 orbits and is ready for Machine Learning modelling. The boundary classes of interest are the Bow shock (SK) and Magnetopause (MP) boundaries~\autoref{tab:labels}.
%\vspace{-0.8cm}
\begin{table}[h!]
    \centering
    \caption{Class labels with their abbreviations and frequency of occurrence.}
    \begin{tabular}{|c|c|c|}\hline
        \textbf{Label} & \textbf{Magnetic Region} & \textbf{Share} \\ \hline
        0 & Interplanetary Magnetic Field (IMF) & $64.8\,\%$ \\ \hline
        1 & Bow Shock Crossing (\textbf{SK}) & $3.7\,\%$ \\ \hline
        2 & Magnetosheath (MSh) & $14.8\,\%$ \\ \hline
        3 & Magnetopause Crossing (\textbf{MP}) & $2.3\,\%$ \\ \hline
        4 & Magnetosphere (MSp) & $14.4\,\%$ \\ \hline
    \end{tabular}
    \label{tab:labels}
\end{table}
%\vspace{-0.8cm}
We assume that the crossing signatures follow a recurring drift theme due to cyclical weather and solar wind conditions, and thus test our approach on this use case where we apply our proposed drift detection algorithm to select the most informative orbits for training and compare that to a equivalent sampling/active learning strategy with random sampling. Preparing annotations in planetary science applications is a labour intense and costly endeavour-- one that can be greatly ameliorated with Active learning methods.
%We theorize that detection of these events are dynamic and we can see them as drifts where the distribution of input features change over time(in this case, mostly due to solar activity) and that we could train an ensemble of classifiers for each distribution, then predict the distribution using concept drift identification and select the classifier for that exact distribution. The underlying notion here is that orbit similarity can be exploited to select the orbits with maximum unseen variation. We take a step further and introduce a more sophisticated active learning method that further reduces the lower bound on required training samples by a significant margin. We evaluate this approach against the existing technique of random sampling and demonstrate a distinct superiority. Preparing annotations in planetary science applications is a labour intense and costly endeavour-- one that can be greatly ameliorated with Active learning methods.

\subsection{Using DriftGAN for sampling orbits}
\label{subsec:application_method}
We follow the assumption that the orbits in the dataset can be grouped into a sets of similar orbits based on their crossing locations and signatures. Upon visual inspection of orbits(~\autoref{fig: example_adjacet_orbits}), it becomes evident that adjacent orbits are likely to be similar to one another with respect to bow shock and magnetopause crossing signatures, while orbits further apart tend to be more different. This pattern appears to have a cyclical nature, where patterns repeat periodically. We exploit this characteristic present in the data, to identify groups with recurring patterns. The hypothesis here is that by identifying groups, we can constrain our sampling to include a fixed size of orbits from each during training to obtain a generalized performance with a significantly lesser amount of training data. This would optimise the sampling strategy with entropy alone~\cite{julkadeep}

We use $B_{z-IMF}$ and $cos\alpha$ to prepare an initial catalogue of similar orbit groups and use those labels to train our drift detectino algorithm. These two features are recognised in literature to maximally influence the orbit charactersitics
Orbit characteristics can be based on several factors, for instance the z-component of the magnetic field in IMF, denoted as $B_{z-IMF}$.  The solar-wind--magnetosphere interaction is particularly sensitive to $B_{z-IMF}$~\cite{and13}, as it determines the state of the magnetosphere, specifically the amount of incoming energy to the magnetosphere and the magnetic flux magnitude on the open field lines.  The cosine of Mercury azimuth angle, denoted as $cos\alpha$~\cite{Sun13}, indicates whether the direction of shock normal is quasi-perpendicular or quasi-parallel to the direction of IMF. The shock conditions principally determine the magnetic signature during a bow shock boundary. We use $B_{z-IMF}$ and $cos\alpha$ to prepare an initial catalogue of similar orbit groups and use those labels to train our drift detection algorithm. These two features are recognised in literature to maximally influence the orbit .

%We use these similarity in features to prepare a first set of groupings for use as labels to train the drift classifier. This classifier then classifies the next stream of orbital data into either of the previously seen groups or a new one. If an orbit is identified to have an unseen distribution, it is assigned a new label.

\begin{figure}[h!tb]%
    \centering
    \subfloat[\centering Orbit \#2923]{{\includegraphics[width = 0.45\linewidth]{images/fig2923.pdf} }}%
    \qquad
    \subfloat[\centering Orbit \#2924]
    {{\includegraphics[width=0.45\linewidth]{images/fig2924.pdf} }}%
     \caption[]{Orbits adjacent to one another are similar in crossing signatures and locations.}
    \label{fig: example_adjacet_orbits}%
\end{figure}

This algorithm can be written down formally as \texttt{$sample\_orbits()$} with parameters $\Omega$ (set of all orbits), $\mathcal{D}$ (set of all drift labels) and $m$ (maximum number of training orbits per drift, hyperparameter) as given in~\autoref{algo:active_learning}.
%\todo{\sj{algo not rendering properly}}
\iffalse
\begin{algorithm}
	\caption{\texttt{sample\_orbits}$(\Omega, \mathcal{D}, k):$}
	\begin{algorithmic}[1]
		\State $\mathcal{T} := \varnothing$ \Comment{Set of training orbits.}\;
		\State $\mathcal{S} := \varnothing$ \Comment{Set of testing orbits.}\;
		\State $d = 1$ \Comment{Current drift label.}\\
		\While{$d \leq |\mathcal{D}|$}
		\State $\mathcal{S} := \mathcal{S} \cup$ \texttt{random.sample}($\Omega_d, |\Omega_d| // 5$)  \Comment{Randomly sample 20\% as testing data.}
		\State $E :=$ \texttt{hash\_table()}
		\For{$\omega \in \Omega_d \backslash \mathcal{S}$} \Comment{Get entropy for all non-testing orbits with current drift.}
		\State $E[\omega] :=$ entropy($\omega$)
		\EndFor
		\State $\mathcal{T} := \mathcal{T} \cup$ \texttt{top\_k}($E, k$) \Comment{Add $k$ most uncertain orbits.}\\
		\State $d := d + 1$ \Comment{Move to the next drift.}
		\EndWhile
		\State \texttt{return} $\mathcal{T}, \mathcal{S}$
	\end{algorithmic}
\end{algorithm}
\fi
\begin{algorithm}
\caption{\texttt{sample\_orbits}$(\Omega, \mathcal{D}, k):$}
     \State $\mathcal{T} := \varnothing$ $\rightarrow$\Comment{Set of training orbits}\;
     \State $\mathcal{S} := \varnothing$ $\rightarrow$\Comment{Set of testing orbits}\;
     \State $d = 1\rightarrow$\Comment{Current drift label.}\;
     \While{$d \leq |\mathcal{D}|$}{
        \State $\mathcal{S} := \mathcal{S} \cup$ \texttt{random.sample}($\Omega_d, |\Omega_d| / 5$) $\rightarrow$ \Comment{Randomly sample 20\% as testing data}\;
        \State $E :=$ \texttt{hash\_table()}\;
        \For{$\omega \in \Omega_d \backslash \mathcal{S}$} {
            \Comment{Get entropy for all non-testing orbits with current drift.}\;
            \State $E[\omega] :=$ entropy($\omega$)\;
        }
        \State $\mathcal{T} := \mathcal{T} \cup$ \texttt{top\_k}($E, k$) $\rightarrow$\Comment{Add $k$ most uncertain orbits}\;
		\State $d := d + 1$ $\rightarrow$\Comment{Move to the next drift}\;
     }
     \State \texttt{return} $\mathcal{T}, \mathcal{S}$\;
\label{algo:active_learning}
\end{algorithm}

\iffalse
 We use the catalogue of detected drifts and sample orbits from them incrementally in an Active learning setting. Within each drift group we rank all the orbits according to an informativeness measure as used in~\cite{julkadeep}.
As our classification model has a series of Multinoulli distributions for output, we measure the orbit uncertainty as a function of the output probabilities using \emph{Shannon entropy} Consider the training set $\mathcal{T} \subseteq \R^{d \times w} \times \{\text{IMF}, \text{SK}, \text{MSh}, \text{MP}, \text{MSp}\}^{w+f}$ with number of features $d \in \N$, window size $w \in \N$. Given a model prediction $\bm{\hat{Y}} = [\bm{\hat{y}}^{(1)}, \dots, \bm{\hat{y}}^{(w)}] \in [0,1]^{5 \times (w)}$, we define its uncertainty as\vspace*{-3mm}
\[
	\uncert(\bm{\hat{Y}}) \coloneqq \max_{j} H(\bm{\hat{y}}^{(j)}) = -\min_{j} \sum_{i = 1}^{5} y^{(j)}_i \log(y^{(j)}_i),\vspace*{-3mm}
\]
where $H: \triangle^4 \to \R$ is the Shannon entropy on the standard $4$-simplex.

To achieve this on the orbit level, we must reduce the individual window uncertainties to a single orbit score. In contrast to the approach in~\cite{julkadeep} who calculate the entropy for only the windows including the crossing labels, we remain agnostic to it and use the entire region to calculate the orbit uncertainty $\hat{f}_{\bm{\theta}}: \R^{d \times w} \to \R^{d \times (w + f)}$ for our task by averaging over all the windows $\widetilde{\mathcal{D}_o}$  as:
\[
	\Uncert_{\hat{f}_{\bm{\theta}}}(\widetilde{\mathcal{D}}_o) \coloneqq \frac{1}{|\widetilde{\mathcal{D}}_o|} \sum_{(\bm{X}, \bm{y}) \in \widetilde{\mathcal{D}}_o} \uncert(\hat{f}_{\bm{\theta}}(\bm{X}))
\]

Using this uncertainty measure, we formulate our active learning procedure in~\autoref{algo:active_learning}. 


%\sj{NOTE: Include the increment function $\increment(n)$ to express how many orbits are added to the training set}

This algorithm can be written down formally as \texttt{$sample\_orbits()$} with parameters $\Omega$ (set of all orbits), $\mathcal{D}$ (set of all drift labels) and $m$ (maximum number of training orbits per drift, hyperparameter) in the following way:

\begin{algorithm}
	\caption{\texttt{sample\_orbits}$(\Omega, \mathcal{D}, m):$}
	\begin{algorithmic}[1]
		\State $\mathcal{T} := \varnothing$ \Comment{Set of training orbits.}
		\State $\mathcal{S} := \varnothing$ \Comment{Set of testing orbits.}
		\State $d = 1$ \Comment{Current drift label.}
		\While{$d \leq |\mathcal{D}|$}
		\State $\mathcal{S} := \mathcal{S} \cup$ \texttt{random.sample}($\Omega_d, |\Omega_d| // 5$)  \Comment{Randomly sample 20\% as \sj{validation/testing data.}}
		\State $E :=$ \texttt{hash\_table()}
		\For{$\omega \in \Omega_d \backslash \mathcal{S}$} \Comment{Get entropy for all non-testing orbits with current drift.}
		\State $E[\omega] :=$ entropy($\omega$)
		\EndFor
		\State $\mathcal{T} := \mathcal{T} \cup$ \texttt{top\_k}($E, m$) \Comment{Add $m$ most uncertain orbits.}
		\State $d := d + 1$ \Comment{Move to the next drift.}
		\EndWhile
		\State \texttt{return} $\mathcal{T}, \mathcal{S}$
	\end{algorithmic}
    \label{algo:active_learning}
\end{algorithm}


To have an augmented set of fixed shaped input vectors and extract aggregated features from them, we use a sliding window, with a stride of size one. 
This is done to ensure translation equivariance \ie the position of the crossing should not matter to the model. 
Hence, the model's input is a window of $w \in \N$ successive time steps, each comprising of $d \in \N$ scalar features. The input windows can thus be expressed as:
\[
    \bm{X} \coloneqq \begin{bmatrix}
       \,\bm{x}^{(1)} & \bm{x}^{(2)} & \cdots & \bm{x}^{(w)}\,
    \end{bmatrix}
    \in \R^{d \times w}
\]


Consequently, the target output matrix of one-hot vectors is $\bm{Y} \in \R^{5 \times (w)}$.

Formally, the classification task is framed as a multi-dimensional multi-class classification: Given the window $\bm{X}$, we predict a sequence of magnetic region probabilities, where each column sums up to one:
\[
    \bm{\hat{Y}} \coloneqq \left[\begin{array}{c c c}
        p_{1,1} & \cdots & p_{1,w}  \\
        \vdots & & \vdots &  \\
        p_{5,1} & \cdots & p_{5,w}  \\
    \end{array}\right] \in [0,1]^{5 \times (w)}
\]

We pass these normalised through a neural network comprised of a convolutional block and a recurrent block, referred to as CRNN\sj{cite}, with the final activations represented as:
$\bm{\gamma}_{\theta}: p_{ij} = \bm{\gamma}_{\theta}(\bm{X})$
where $\bm{\gamma}$ is the CRNN model, with $\theta$ as its parameters. 
\fi
%\cf{Need to find a soft stop instead of hard stop}




==> content/application_mercury.tex <==


%\section{Towards active learning for detection bow shock and mangetopause crossings around Mercury}

We apply our approach to a real use case from planetary science to demonstrate its applicability as an improved sampling strategy.


\subsection{Use case description}
\sj{You can massively shorten the introduction and refer to this image describing the use case}
\begin{figure}[ht]
    \centering
    \subfloat[\centering ]{{\includegraphics[width=5cm, height=3cm]{images/slavin_mercury.jpg} }}%
    \qquad
    \subfloat[\centering]
    {{\includegraphics[width=5cm, height = 3cm]{images/zurbuchen_messenger.jpg} }}%
     \caption[]{{(a) Schematic view of Mercury's magnetic conditions~\cite{slavin2004mercury}.The bow shock slows down the approaching solar wind to subsonic speeds. The magnetopause further acts as an obstacle.  (b) A typical MESSENGER orbit path: the spacecraft passed from
    the \emph{interplanetary magnetic field} (IMF) through bow shock, magnetosheath, magnetopause and magnetosphere regions of Mercury and then through the same sequence in reverse~\cite{zurbuchen2011messenger}. }}
    \label{fig: introduction}%
\end{figure}

The \emph{magnetosphere} of a planet is the area surrounding it where the planet's magnetic field is stronger than that of the surrounding interplanetary space. 
The \emph{magnetopause} is the outer boundary of this region, while the \emph{magnetosheath} lies above it and extends to the bow shock. 
The \emph{bow shock} is a shock wave that decelerates the solar wind and deflects it around the planet's magnetospheric cavity~(C.f~\autoref{fig: introduction}). 
Studying magnetic fields of planets has been a long standing interest in planetary science. For Mercury, the innermost planet in our solar system, the magnetic field is peculiar: one, it is extremely weak-- about 1~\% that of the Earth, second, due to its close proximity to the sun, is heavily influenced by the varying solar wind conditions, and thus very dynamic. Studying such magnetospheres can yield interesting insights into more complex magnetospheres such as the Earth's. In such pursuit, NASA launched a spacecraft called MESSENGER to orbit Mercury and conduct long-term empirical studies\cite{solomon2007messenger}. MESSENGER collected over 8000 incidents of bow shock and magnetopause crossings during its four-year journey from 2011 to 2015, due to the relatively small size of Mercury's magnetosphere compared to Earth's.

However, since supervised learning typically requires a large number of samples for training, they also proposed an active learning approach to select the most informative orbits using an entropy criterion. The underlying notion here is that orbit similarity can be exploited to select the orbits with maximum unseen variation. We take a step further and introduce a more sophisticated active learning method that further reduces the lower bound on required training samples by a significant margin. We evaluate this approach against the existing technique and random and demonstrate a distinct superiority. Preparing annotations in planetary science applications is a labour intense and costly endeavour-- one that can be greatly ameliorated with Active learning methods.

The dataset we use for our experiments in this work contains magnetic field measurements from the MESSENGER magnetometer instrument. The data is already preprocessed with removal of calibration signals, enrichment with Mercury position data, and split according to UTC day boundaries and Mercury apoapsis. This cleaned and prepared dataset introduced in~\cite{julkadeep} contains 2776 orbits and is ready for Machine Learning modelling. The final annotations that have been derived from the work of~\cite{philpott2020shape} have finally a class distribution given in in~\Cref{tab:labels}. The boundary classes of interest are the Bow shock (SK) and Magnetopause (MP) boundaries.

\begin{table}[h!]
    \centering
    \caption{Class labels with their abbreviations and frequency of occurence. The boundary classes are highly underrepresented. Classification involves accurately detecting these relatively rare events.}
    \begin{tabular}{ r || l | r }\hline
    \textbf{label} & \textbf{magnetic region} & \textbf{share} \\\hhline{|=||=|=|}
        0 & interplanetary magnetic field (IMF) & $64.8\,\%$ \\\hline
        1 & bow shock crossing (\textbf{SK}) & $3.7\,\%$ \\\hline
        2 & magnetosheath (MSh) & $14.8\,\%$ \\\hline
        3 & magnetopause crossing (\textbf{MP}) & $2.3\,\%$ \\\hline
        4 & magnetosphere (MSp) & $14.4\,\%$ \\\hline
    \end{tabular}

    \label{tab:labels}
\end{table}


We follow the assumption that the orbits in the dataset can be grouped into a sets of similar orbits based on their crossing locations and signatures. Upon visual inspection of orbits [CLEVERREF NOT WORKING], it becomes evident that adjacent orbits are likely to be similar to one another with respect to bow shock and magnetopause crossing signatures, while orbits further apart tend to be more different. This pattern appears to have a cyclical nature, where patterns repeat periodically. We exploit this characteristic present in the data, to identify groups with recurring patterns. The hypothesis here is that by identifying groups, we can constrain our sampling to include a fixed size of orbits from each during training to obtain a generalisable performance with a significantly lesser amount of training data. This would optimise the sampling strategy with entropy alone~\cite{julkadeep}
Orbit characteristics can be based on several factors, for instance the z-component of the magnetic field in IMF, denoted as $B_{z-IMF}$.  The solar-wind--magnetosphere interaction is particularly sensitive to $B_{z-IMF}$~\cite{and13}, as it determines the state of the magnetosphere, specifically the amount of incoming energy to the magnetosphere and the magnetic flux magnitude on the open field lines.  The cosine of Mercury azimuth angle, denoted as $cos\alpha$~\cite{Sun13}, indicates whether the direction of shock normal is quasi-perpendicular or quasi-parallel to the direction of IMF. The shock conditions principally determine the magnetic signature during a bow shock boundary. We use these similarity in features to prepare a first set of groupings for use as labels to train the drift classifier. This classifier then classifies the next stream of orbital data into either of the previously seen groups or a new one. If an orbit is identified to have an unseen distribution, it is assigned a new label.

\begin{figure}[h!tb]%
    \centering
    \subfloat[\centering Orbit \#2923]{{\includegraphics[width = 0.45\linewidth]{images/fig2923.pdf} }}%
    \qquad
    \subfloat[\centering Orbit \#2924]
    {{\includegraphics[width=0.45\linewidth]{images/fig2924.pdf} }}%
     \caption[]{Orbits adjacent to one another are similar in crossing signatures and locations.}
    \label{fig: example_adjacet_orbits}%
\end{figure}


NOTE: We change the algorithm to expect recurring drifts.


The drift detection algorithm can be formally defined as \texttt{detect\_drifts()}~(C.f\Cref{alg: alg1}) with parameters $d_{gen}$ (generator label), $\mathcal{O}$ (sequential set of unlabelled orbits), $\mathcal{D}_{init}$ (hash table of initial orbit groupings with orbit numbers and drift labels):
\begin{algorithm}[h]
	\label{alg: alg1}
	\caption{\texttt{detect\_drifts}$(d_{gen}, \mathcal{O}, \mathcal{D}_{init} : \mathbb{R}^{d\times w}\rightarrow \mathbb{R}^{d_{gen}}):$}
	\begin{algorithmic}[1]
		\State $\mathcal{D} := \mathcal{D}_{init}$ \Comment{Hash map of orbits and drift labels.}
		\State $gen :=$ \texttt{Generator()} $: \mathbb{R}^{d\times w}\rightarrow \mathbb{R}^{d\times w}$ \Comment{Generator.}
		\State $dis :=$ \texttt{Discriminator()} $: \mathbb{R}^{d\times w}\rightarrow \mathbb{R}^{|\mathcal{D}|}$ \Comment{Discriminator.}
		\State $\mathcal{T} := $ \texttt{create\_training\_dataset$(\mathcal{O}, \mathcal{D})$} \Comment{Labelled training orbits.}
		\State $\mathcal{T}_{gen} := $ \texttt{equalise\_and\_concatenate$(\mathcal{T})$} \Comment{Training data for generator.}
		\State $dis :=$ \texttt{train\_discriminator$(\mathcal{T}, dis, gen, d_{gen})$} \Comment{Initial training.}
		\State $gen :=$ \texttt{train\_generator$(\mathcal{T}_{gen}, dis, gen, d_{gen})$}
		\State $i := 0$ \Comment{Current orbit number.}
		
		\While{$i < |\mathcal{O}|$}
		\State $d := dis(\mathcal{O}_i)$ \Comment{Get most probable drift label from discriminator.} 
		\If{$d \in [\mathcal{D}_1 : \mathcal{D}_{|j|}]$}
		\State \texttt{reset\_top\_layer$(dis)$} \Comment{Reset the top \texttt{Linear} layer.}
		    
		\Else
		\State \texttt{update$(dis)$} \Comment{Reset the top \texttt{Linear} layer and increase its output size by 1.}
		\State $d_{gen} = d_{gen} + 1$
		    
		\EndIf
		    
		\State $n = 1$ \Comment{Number of adjacent orbits in a drift.}
		    
		\If{$d \neq \mathcal{D}[i-1]$}
		\State $n =$ 14
		    
		\EndIf
		    
		\State $j := 0$
		    
		\While{$j < n$}
		\State $\mathcal{D}[\mathcal{O}_{i+j}] := d$ \Comment{Assign drift label to orbits.}
		\State $j := j + 1$
		\EndWhile
		\State $\mathcal{T} := $ \texttt{create\_training\_dataset$(\mathcal{O}, \mathcal{D})$} \Comment{Dataset with new drift.}
		\State $\mathcal{T}_{gen} := $ \texttt{equalise\_and\_concatenate$(\mathcal{T})$}
		\State $dis :=$ \texttt{train\_discriminator$(\mathcal{T}, dis, gen, d_{gen})$}
		\State $gen :=$ \texttt{train\_generator$(\mathcal{T}_{gen}, dis, gen, d_{gen})$}
		\State $i := i + n$ \Comment{Move to the next unlabelled orbit.}
		\EndWhile
		\State \texttt{return} $\mathcal{D}$
	\end{algorithmic}
 \end{algorithm}


 We use the catalogue of detected drifts and sample orbits from them incrementally in an Active learning setting. Within each drift group we rank all the orbits according to an informativeness measure as used in~\cite{julkadeep}.
As our classification model has a series of Multinoulli distributions for output, we measure the orbit uncertainty as a function of the output probabilities using \emph{Shannon entropy} Consider the training set $\mathcal{T} \subseteq \R^{d \times w} \times \{\text{IMF}, \text{SK}, \text{MSh}, \text{MP}, \text{MSp}\}^{w+f}$ with number of features $d \in \N$, window size $w \in \N$. Given a model prediction $\bm{\hat{Y}} = [\bm{\hat{y}}^{(1)}, \dots, \bm{\hat{y}}^{(w)}] \in [0,1]^{5 \times (w)}$, we define its uncertainty as\vspace*{-3mm}
\[
	\uncert(\bm{\hat{Y}}) \coloneqq \max_{j} H(\bm{\hat{y}}^{(j)}) = -\min_{j} \sum_{i = 1}^{5} y^{(j)}_i \log(y^{(j)}_i),\vspace*{-3mm}
\]
where $H: \triangle^4 \to \R$ is the Shannon entropy on the standard $4$-simplex.

% ~\footnote{\( \triangle^{n-1} \coloneqq \{(p_1, p_2, \dots, p_n) \in \R^n \mid \forall i: p_i \ge 0, \sum_{i = 1}^{n}p_i = 1\} \subseteq [0, 1]^n\)}.

To achieve this on the orbit level, we must reduce the individual window uncertainties to a single orbit score. In contrast to the approach in~\cite{julkadeep} who calculate the entropy for only the windows including the crossing labels, we remain agnostic to it and use the entire region to calculate the orbit uncertainty $\hat{f}_{\bm{\theta}}: \R^{d \times w} \to \R^{d \times (w + f)}$ for our task by averaging over all the windows $\widetilde{\mathcal{D}_o}$  as:
\[
	\Uncert_{\hat{f}_{\bm{\theta}}}(\widetilde{\mathcal{D}}_o) \coloneqq \frac{1}{|\widetilde{\mathcal{D}}_o|} \sum_{(\bm{X}, \bm{y}) \in \widetilde{\mathcal{D}}_o} \uncert(\hat{f}_{\bm{\theta}}(\bm{X}))
\]

Using this uncertainty measure, we formulate our active learning procedure in~\autoref{algo:active_learning}. 
% Instead of strictly adding orbits one-by-one, we more generally allow for an \emph{increment function} $\increment: \N_0 \to \N$ that dictates the number of most uncertain orbits to add, depending on the number of already seen orbits. 

\sj{NOTE: Include the increment function $\increment(n)$ to express how many orbits are added to the training set}

This algorithm can be written down formally as \texttt{sample\_orbits()} with parameters $\Omega$ (set of all orbits), $\mathcal{D}$ (set of all drift labels) and $m$ (maximum number of training orbits per drift, hyperparameter) in the following way:

\begin{algorithm}
	\caption{\texttt{sample\_orbits}$(\Omega, \mathcal{D}, m):$}
	\begin{algorithmic}[1]
		\State $\mathcal{T} := \varnothing$ \Comment{Set of training orbits.}
		\State $\mathcal{S} := \varnothing$ \Comment{Set of testing orbits.}
		\State $d = 1$ \Comment{Current drift label.}
		\While{$d \leq |\mathcal{D}|$}
		\State $\mathcal{S} := \mathcal{S} \cup$ \texttt{random.sample}($\Omega_d, |\Omega_d| // 5$)  \Comment{Randomly sample 20\% as \sj{validation/testing data.}}
		\State $E :=$ \texttt{hash\_table()}
		\For{$\omega \in \Omega_d \backslash \mathcal{S}$} \Comment{Get entropy for all non-testing orbits with current drift.}
		\State $E[\omega] :=$ entropy($\omega$)
		\EndFor
		\State $\mathcal{T} := \mathcal{T} \cup$ \texttt{top\_k}($E, m$) \Comment{Add $m$ most uncertain orbits.}
		\State $d := d + 1$ \Comment{Move to the next drift.}
		\EndWhile
		\State \texttt{return} $\mathcal{T}, \mathcal{S}$
	\end{algorithmic}
\end{algorithm}


To have an augmented set of fixed shaped input vectors and extract aggregated features from them, we use a sliding window, with a stride of size one. 
This is done to ensure translation equivariance \ie the position of the crossing should not matter to the model. 
Hence, the model's input is a window of $w \in \N$ successive time steps, each comprising of $d \in \N$ scalar features. The input windows can thus be expressed as:
\[
    \bm{X} \coloneqq \begin{bmatrix}
       \,\bm{x}^{(1)} & \bm{x}^{(2)} & \cdots & \bm{x}^{(w)}\,
    \end{bmatrix}
    \in \R^{d \times w}
\]

Consquently, the target output matrix of one-hot vectors is $\bm{Y} \in \R^{5 \times (w)}$.

Formally, the classification task is framed as a multi-dimensional multi-class classification: Given the window $\bm{X}$, we predict a sequence of magnetic region probabilities, where each column sums up to one:
\[
    \bm{\hat{Y}} \coloneqq \left[\begin{array}{c c c}
        p_{1,1} & \cdots & p_{1,w}  \\
        \vdots & & \vdots &  \\
        p_{5,1} & \cdots & p_{5,w}  \\
    \end{array}\right] \in [0,1]^{5 \times (w)}
\]

We pass these normalised through a neural network comprised of a convolutional block and a recurrent block, referred to as CRNN\sj{cite}, with the final activations represented as:
$\bm{\gamma}_{\theta}: p_{ij} = \bm{\gamma}_{\theta}(\bm{X})$
where $\bm{\gamma}$ is the CRNN model, with $\theta$ as its parameters. 


\begin{table}[h!tb]
\centering
\caption{CRNN performance our approach vs benchmark. Trained on 278 sampled orbits and tested on 97 orbits.\textbf{ALD} denotes Active Learning with Drift detection (our approach). \textbf{AD} denotes Active Learning without drift detection. All values are rounded to two decimals. Best values are marked in bold.}
%\vspace*{0.5mm}
  \begin{tabular}{l||p{0.6cm}p{0.6cm}|p{0.6cm}p{0.6cm}|p{0.6cm}p{0.6cm}|p{0.6cm}p{0.6cm}|p{0.6cm}p{0.6cm}|p{0.6cm}p{0.6cm}}
    
    \toprule
    \multirow{2}{*}{} &
      \multicolumn{2}{c}{\textbf{IMF}} &
      \multicolumn{2}{c}{\textbf{SK}} &
      \multicolumn{2}{c}{\textbf{MSh}} &
      \multicolumn{2}{c}{\textbf{MP}} &
      \multicolumn{2}{c}{\textbf{MSp}} &
      \multicolumn{2}{c}{\textbf{Average}}
      \\\hhline{ |=|=|=|=|=|=|=|=|=|=|=|=|=} 
      & {ALD} & {AL} & {ALD} & {AL} & {ALD} & {AL} & {ALD} & {AL} & {ALD} & {AL}& {ALD} & {AL}\\
      \midrule
    \textbf{F1} & \bm{0.98} & 0.93 & \bm{0.66} & 0.5  & 0.86 & 0.86 & 0.626 & \bm{0.64} & \bm{0.99} & 0.93 & \bm{0.82} & 0.78\\
    \textbf{Recall} & \bm{0.97} & 0.95 & \bm{0.73} & 0.71 & \bm{0.85} & 0.84 & 0.645 & \bm{0.76} & \bm{0.95} & 0.89& 0.83 & 0.83  \\
    \textbf{Precision} & \bm{0.98} & 0.92 & \bm{0.59} & 0.39 & 0.88 & \bm{0.88}  & \bm{0.61} & 0.56 & \bm{0.98} & 0.93 & \bm{0.80} & 0.74 \\
    \bottomrule
  \end{tabular}
  \label{tab: benchmark_comparison}
\end{table}


\begin{table}[h!tb]
\centering
\vspace*{1mm}
\caption{CRNN performance Random Sampling. The number of training orbits is 278, like in table 2 to compare active learning against random sampling }

\begin{tabular}{l||r|r|r|r|r}\hline
	\textbf{} & \textbf{IMF} & \textbf{SK} & \textbf{MSh} & \textbf{MP} &\textbf{MSp}\\\hhline{=#=|=|=|=|=} 
	\textbf{F1} & 0.718\ & 0.397\ & 0.518\ & 0.457\ & 0.780\ \\\hline
	\textbf{Recall} & 0.592\ & 0.442\ & 0.531\ & 0.494\ &0.959\ \\\hline
    \textbf{Precision} & 0.912\ & 0.361\ & 0.506\ & 0.425\ &0.658\ \\\hline
\end{tabular}
\label{tab:test_eval}
\vspace*{-1mm}
\end{table}
